Boltzmann Meets Lorentz: A Surrogate Model for Black Hole Echoes

The existence of black hole horizons has not been strictly proven observationally, and indeed it may not be possible to do so. However, alternatives may be established by the observation of gravitational wave echoes that probe possible near-horizon structure. These echoes are proposed to be generated in exotic compact objects that are horizonless and feature a partially reflecting "wall" inside their light rings, creating a cavity in which gravitational perturbations may echo, while leaking out through the angular momentum barrier with each pass. The characteristic signature of echoes is a comb of nearly evenly spaced spectral resonances. While approximately true, deviations from this simple picture can lead to severe observational signal losses. In this paper, we explore such subtleties with the latest results for echo sourcing and geometry. A physically motivated echo model is then developed as a sum over Lorentzian spectral lines, parametrized by functions of the horizon frame frequency and the size of the cavity. Our final spectrum is a function of only the mass and spin of the black hole, as well as the UV scale of the near-horizon physics. We then apply this model in a search for echoes in the gravitational wave event with the loudest ringdown signal in LIGO/Virgo, i.e. GW190521. We interpret our findings as a measurement of the fractional energy in post-merger echoes equal to $E_{echoes} / E_{GR} = 8.9 \pm 4.5\%$, where the uncertainty range represents the 90% credible region. The robustness of this result is tested against noise backgrounds and simulated injections, and we find that a signal persists through modifications to the model and changes in the data search.

==> ExtraPlots.tex <==
%\section{Plots}

%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{LongTimeBoltzEchoSearchMassA2.pdf}
%\caption{\label{fig:LongTimeBoltzEchoSearchMassA2} The same but arranged by mass.}
%\end{figure}
%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{LongTimeBoltzEchoSearchHistA2.pdf}
%\caption{\label{fig:LongTimeBoltzEchoSearchHistA2} A histogram of SNRs for the $\alpha = 2$ Boltzmann model using the $120s$ time segment.}
%\end{figure}
%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{LongTimeBoltzEchoSearchHistCumA2.pdf}
%\caption{\label{fig:LongTimeBoltzEchoSearchHistCumA2} The cumulative $\alpha = 2$ long-time histogram.}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{LongTimeBoltzEchoSearchMass.pdf}
%\caption{\label{fig:LongTimeBoltzEchoSearchMass} The same as the previous plot but arranged by increasing mass.}
%\end{figure}
%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{LongTimeBoltzEchoSearchHist.pdf}
%\caption{\label{fig:LongTimeBoltzEchoSearchHist} A histogram of SNRs for the standard Boltzmann model using the $120s$ time segment.}
%\end{figure}
%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{LongTimeBoltzEchoSearchHistCum.pdf}
%\caption{\label{fig:LongTimeBoltzEchoSearchHistCum} The cumulative long-time histogram.}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{LongTimeBoltz.pdf}
%\caption{\label{fig:LongTimeBoltz} Most echo searches in the literature are done over short durations of time, since it is expected that the decay rate for each echo is sufficiently large to quickly cause noise to increase faster than signal for current detectors. One method, however, requires timescales an order of magnitude greater than the norm.[[CITE WINDOWS AND BOB]] The motivation for this is to sharpen resonances by increasing frequency resolution, and to increase their height by including more echoes. In this plot, we show the standard Boltzmann model overlaid on the data all resolved from a timescale of $T = 120s$ instead of the usual $15s$.}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{EchoDatSearchBoltzA1Hist.pdf}
%\caption{\label{fig:EchoDatSearchBoltzA1Hist} A histogram of the SNR values measured using the standard Boltzmann model and a 15s segment for 23896 sets of $(a,M)$ parameters for the echo search (this is somewhat lower resolution than the plot of SNR as a function of spin/mass, but with qualitatively equivalent results).}
%\end{figure}
%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{EchoDatSearchBoltzA1HistCum.pdf}
%\caption{\label{fig:EchoDatSearchBoltzA1HistCum} A cumulative histogram of the same.}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{BackMaxSNR.pdf}
%\caption{\label{fig:BackMaxSNR} The standard Boltzmann echo search gave a maximum SNR of 12, showing a peak distinctly rising above the surrounding noise. To assess the significance of this, we compared to 100 sets of data prior to the event (meaning with no echoes). This plot gives the maximum SNR from the data search done for each background. The x-axis marks the index of the data segment where the first segment is at a GPS time of $t_{event} - 2000$. Subsequent data segments were taken at 20s intervals, and the search itself was done using the first 15s of each set of 20s of data. These results demonstrate that SNRs of equal or greater magnitude to the observed signal can be present in 2 out of 100 backgrounds, leading to a significance of about $2.3\sigma$.}
%\end{figure}
%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{BackParameterDist.pdf}
%\caption{\label{fig:BackParameterDist} The mass and spin values at the maximum SNR for each background search. The density of points is somewhat clustered around the LIGO best-fit parameters of $a = 0.72$ and $M \approx 258$, where $M$ here is the redshifted mass. The value of 258 was obtained from the best-fit redshift by taking $M = 1.82*142 = 258$. This clustering may be the result of the Monte Carlo chains being more dense for more likely parameter ranges.}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{MinSub.png}
%\caption{\label{fig:MinSub} Caption fill.}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{MinSubModelComp.png}
%\caption{\label{fig:MinSubModelComp} Caption fill.}
%\end{figure}

%In Fig.\ref{fig:SNRDensity} we provide a density plot of the SNR as a function of mass and spin for a search immediately after the main GW event.
%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{SNRDensity.png}
%\caption{\label{fig:SNRDensity} The signal to noise ratio as a function of mass and spin for GW190521 with the Boltzmann model for echoes. The data ranges are centered about the best fit values, and are representative of the LIGO 90\% confidence intervals, with the exception of a slightly lower mass limit chosen for visualization. The black dashed lines mark the best fit values. The SNR at lower spins appears relatively stretched as a result of nonlinear advancement of the horizon frequency as a function of spin.}
%\end{figure}
%The stretching of the SNR as a function of spin is due to the nonlinearity of the horizon frequency, shown in Fig.\ref{fig:w0T}.
%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{w0T.png}
%\caption{\label{fig:w0T} The data used for each SNR calculation is centered about the horizon frequency $w0$. Here the nonlinearity in $w0$ is shown by plotting the difference between values as a function of spin. [[W0 VS $\omega$ 0 CARE ON NOTATION!!]]}
%\end{figure}
%[[SNR vs S/N notation]].

%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{BackLikelihood.pdf}
%\caption{\label{fig:BackLikelihood} The likelihood function calculated according to [[INSERT REFERENCE]] for each of the 100 background searches. This is strongly correlated with the maximum SNR shown in [[REFERENCE FIGURE]].}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{InjEvSNRFixed.pdf}
%\caption{\label{fig:InjEvSNRFixed} In addition to performing 100 background checks on data where it was known that echoes were not present, we also tested the model against simulated injections where the echo model at the best-fit spin was injected into noise. This plot shows the energy of the injection as a function of maximum SNR, for 100 total injections. This information was sufficient to approximate the result as a linear function giving the energy of echoes as a function of maximum SNR.}
%\end{figure}
%\begin{figure}
%\centering
%\includegraphics[width=0.47\textwidth]{MeasuredEnergyInjResiduals.pdf}
%\caption{\label{fig:MeasuredEnergyInjResiduals} From the series of 100 simulated injections of echoes into a background set of noise, a linear model was created of energy as a function of SNR with residuals plotted here.}
%\end{figure}
